git2net - Mining Time-Stamped Co-Editing Networks from Large git Repositories

Data from software repositories have become an important foundation for the empirical study of software engineering processes. A recurring theme in the repository mining literature is the inference of developer networks capturing e.g. collaboration, coordination, or communication from the commit history of projects. Most of the studied networks are based on the co-authorship of software artefacts defined at the level of files, modules, or packages. While this approach has led to insights into the social aspects of software development, it neglects detailed information on code changes and code ownership, e.g. which exact lines of code have been authored by which developers, that is contained in the commit log of software projects. Addressing this issue, we introduce git2net, a scalable python software that facilitates the extraction of fine-grained co-editing networks in large git repositories. It uses text mining techniques to analyse the detailed history of textual modifications within files. This information allows us to construct directed, weighted, and time-stamped networks, where a link signifies that one developer has edited a block of source code originally written by another developer. Our tool is applied in case studies of an Open Source and a commercial software project. We argue that it opens up a massive new source of high-resolution data on human collaboration patterns.

==> tools/tools_entity_relationship_diagrams.tex <==
\def\ReplaceStr#1{%
	\IfSubStr{#1}{ }{%
		\StrSubstitute{#1}{ }{\_}}{#1}}

\makeatletter
    \pgfarrowsdeclare{crow's foot}{crow's foot}
    {
        \pgfarrowsleftextend{+-.5\pgflinewidth}%
        \pgfarrowsrightextend{+.5\pgflinewidth}%
    }
    {
        \pgfutil@tempdima=0.6pt%
        %\advance\pgfutil@tempdima by.25\pgflinewidth%
        \pgfsetdash{}{+0pt}%
        \pgfsetmiterjoin%
        \pgfpathmoveto{\pgfqpoint{0pt}{-5\pgfutil@tempdima}}%
        \pgfpathlineto{\pgfqpoint{-10\pgfutil@tempdima}{0pt}}%
        \pgfpathlineto{\pgfqpoint{0pt}{5\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{-6pt}{-4pt}}%
        \pgfpathlineto{\pgfqpoint{-6pt}{-4pt}}%
        \pgfpathlineto{\pgfqpoint{-6pt}{4pt}}%
        \pgfusepathqstroke%
    }

    \pgfarrowsdeclare{omany}{omany}
    {
        \pgfarrowsleftextend{+-.5\pgflinewidth}%
        \pgfarrowsrightextend{+.5\pgflinewidth}%
    }
    {
        \pgfutil@tempdima=0.6pt%
        %\advance\pgfutil@tempdima by.25\pgflinewidth%
        \pgfsetdash{}{+0pt}%
        \pgfsetmiterjoin%
        \pgfpathmoveto{\pgfqpoint{0pt}{-5\pgfutil@tempdima}}%
        \pgfpathlineto{\pgfqpoint{-10\pgfutil@tempdima}{0pt}}%
        \pgfpathlineto{\pgfqpoint{0pt}{5\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{-6pt}{-6pt}}%
        \pgfpathcircle{\pgfpoint{-9pt}{0}}{3pt}%\pgfusepath{fill=white}
        \pgfusepathqstroke%
    }

    \pgfarrowsdeclare{one}{one}
    {
        \pgfarrowsleftextend{+-.5\pgflinewidth}%
        \pgfarrowsrightextend{+.5\pgflinewidth}%
    }
    {
        \pgfutil@tempdima=0.6pt%
        %\advance\pgfutil@tempdima by.25\pgflinewidth%
        \pgfsetdash{}{+0pt}%
        \pgfsetmiterjoin%
        \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{-3pt}{-4pt}}%
        \pgfpathlineto{\pgfqpoint{-3pt}{-4pt}}%
        \pgfpathlineto{\pgfqpoint{-3pt}{4pt}}%
        \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{-5pt}{-4pt}}%
        \pgfpathlineto{\pgfqpoint{-5pt}{-4pt}}%
        \pgfpathlineto{\pgfqpoint{-5pt}{4pt}}%
        \pgfusepathqstroke%
    }
    \pgfarrowsdeclare{oone}{oone}
    {
        \pgfarrowsleftextend{+-.5\pgflinewidth}%
        \pgfarrowsrightextend{+.5\pgflinewidth}%
    }
    {
        \pgfutil@tempdima=0.6pt%
        %\advance\pgfutil@tempdima by.25\pgflinewidth%
        \pgfsetdash{}{+0pt}%
        \pgfsetmiterjoin%
        \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{-4pt}{-4pt}}%
        \pgfpathlineto{\pgfqpoint{-4pt}{-4pt}}%
        \pgfpathlineto{\pgfqpoint{-4pt}{4pt}}%
        \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{-6pt}{-6pt}}%
        \pgfpathcircle{\pgfpoint{-9pt}{0}} {3pt}
        \pgfusepathqstroke%
    }
    \makeatother

    \tikzset{
        entity/.code={
            \tikzset{
                % label=above:#1,
                name=#1,
                inner ysep=1mm,
                inner xsep=0mm,
                every entity/.try,
                fill=white,
                rounded corners,
                very thick,
                % rectangle split,
                % rectangle split parts=2,
                % general shadow={
                %     shadow xshift=0.0625in,
                %     shadow yshift=-0.0625in,
                %     opacity=0.5,
                %     fill=black!50
                % }
            }%
            \def\entityname{#1}%
        },
        entity anchor/.style={matrix anchor=#1.center},
        every entity/.style={
                draw,
        },
        every property/.style={
            inner xsep=.1cm, inner ysep=0.05cm, anchor=west, text width=3.3cm
        },
        zig zag to/.style={
            rounded corners,
            to path={(\tikztostart) -| ($(\tikztostart)!#1!(\tikztotarget)$) |- (\tikztotarget) \tikztonodes}
        },
        zig zag to/.default=0.5,
        one to one/.style={
            one-one, zig zag to, thick
        },
        one to oone/.style={
            one-oone, zig zag to, thick
        },
        one to many/.style={
            one-crow's foot, zig zag to, thick
        },
        one to omany/.style={
            one-omany, zig zag to, thick
        },
        oone to one/.style={
            oone-one, zig zag to, thick
        },
        oone to oone/.style={
            oone-oone, zig zag to, thick
        },
        oone to many/.style={
            -crow's foot, dashed, zig zag to, thick
        },
        oone to omany/.style={
            -omany, dashed, zig zag to, thick
        },
        many to one/.style={
            crow's foot-one, zig zag to, thick
        },
        many to oone/.style={
            crow's foot-, dashed, zig zag to, thick
        },
        many to many/.style={
            crow's foot-crow's foot, zig zag to, thick
        },
        many to omany/.style={
            crow's foot-omany, zig zag to, thick
        },
        omany to one/.style={
            omany-one, zig zag to, thick
        },
        omany to oone/.style={
            omany-, dashed, zig zag to, thick
        },
        omany to many/.style={
            omany-crow's foot, zig zag to, thick
        },
        omany to omany/.style={
            omany-omany, zig zag to, thick
        },
    }

    \def\property#1{\node[name=\entityname-#1, every property/.try]{#1};}
    \def\properties{\begingroup\catcode`\_=11\relax\processproperties}
    \def\processproperties#1{\endgroup%
        \def\propertycode{}%
        \foreach \p in {#1}{%
            \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter\propertycode%
                \expandafter\expandafter\expandafter{\expandafter\propertycode\expandafter\property\expandafter{\p}\\}%
        }%
        \propertycode%
    }

    \def\str#1#2{
        \node[name=\entityname-#1, every property/.try]{\scalebox{.75}[.75]{\footnotesize#2#1}};
        \node[name=\entityname-#1, every property/.try, text width=3.3cm, 
        align=right]{\textcolor{black!50}{\scalebox{.75}[.75]{\scriptsize\textit{str}}}};\\
    }
    \def\int#1#2{
        \node[name=\entityname-#1, every property/.try]{\scalebox{.75}[.75]{\footnotesize #2#1}};
        \node[name=\entityname-#1, every property/.try, red, text width=3.3cm, 
        align=right]{\textcolor{black!50}{\scalebox{.75}[.75]{\scriptsize\textit{int}}}};\\
    }
    \def\float#1#2{
        \node[name=\entityname-#1, every property/.try]{\scalebox{.75}[.75]{\footnotesize#2#1}};
        \node[name=\entityname-#1, every property/.try, red, text width=3.3cm, 
        align=right]{\textcolor{black!50}{\scalebox{.75}[.75]{\scriptsize\textit{float}}}};\\
    }
%    \def\list#1#2{
%        \node[name=\entityname-#1, every property/.try]{\scalebox{.75}[.75]{\footnotesize#2#1}};
%        \node[name=\entityname-#1, every property/.try, red, text width=3.3cm, 
%        align=right]{\textcolor{black!50}{\scalebox{.75}[.75]{\scriptsize\textit{list}}}};\\
%    }
    \def\date#1#2{
        \node[name=\entityname-#1, every property/.try]{\scalebox{.75}[.75]{\footnotesize#2#1}};
        \node[name=\entityname-#1, every property/.try, red, text width=3.3cm, 
        align=right]{\textcolor{black!50}{\scalebox{.75}[.75]{\scriptsize\textit{date}}}};\\
    }
    \def\bool#1#2{
        \node[name=\entityname-#1, every property/.try]{\scalebox{.75}[.75]{\footnotesize#2#1}};
        \node[name=\entityname-#1, every property/.try, red, text width=3.3cm, 
        align=right]{\textcolor{black!50}{\scalebox{.75}[.75]{\scriptsize\textit{bool}}}};\\
    }
    \def\key#1#2{
        \node[name=\entityname-#1, every property/.try]{\scalebox{.75}[.75]{\footnotesize#2#1}};
        \node[name=\entityname-#1, every property/.try, red, text width=3.3cm, 
        align=right]{\textcolor{black!50}{\scalebox{.75}[.75]{\scriptsize\textit{KEY}}}};\\
    }
    \def\TODO#1#2{
        \node[name=\entityname-#1, every property/.try]{\scalebox{.75}[.75]{\footnotesize#2#1}};
        \node[name=\entityname-#1, every property/.try, red, text width=3.3cm, 
        align=right]{\textcolor{black!50}{\scalebox{.75}[.75]{\scriptsize\textbf{TODO}}}};\\
    }

    \def\entitynamenode{%
    \node[every entity name/.try] (\entityname-name) {\scriptsize\MakeUppercase{\textbf{\entityname}}};
    \draw[thick, shorten <= 1mm, shorten >= 1mm] (\entityname-name.south west) -- (\entityname-name.south east);
    \\[1ex]
    }
    \tikzset{
      every entity name/.style={every property/.try, align=center, text 
      width=3.3cm}
    }
